MBDS: A Multi-Body Dynamics Simulation Dataset for Graph Networks Simulators

Modeling the structure and events of the physical world constitutes a fundamental objective of neural networks. Among the diverse approaches, Graph Network Simulators (GNS) have emerged as the leading method for modeling physical phenomena, owing to their low computational cost and high accuracy. The datasets employed for training and evaluating physical simulation techniques are typically generated by researchers themselves, often resulting in limited data volume and quality. Consequently, this poses challenges in accurately assessing the performance of these methods. In response to this, we have constructed a high-quality physical simulation dataset encompassing 1D, 2D, and 3D scenes, along with more trajectories and time-steps compared to existing datasets. Furthermore, our work distinguishes itself by developing eight complete scenes, significantly enhancing the dataset's comprehensiveness. A key feature of our dataset is the inclusion of precise multi-body dynamics, facilitating a more realistic simulation of the physical world. Utilizing our high-quality dataset, we conducted a systematic evaluation of various existing GNS methods. Our dataset is accessible for download at https://github.com/Sherlocktein/MBDS, offering a valuable resource for researchers to enhance the training and evaluation of their methodologies.

==> ICIC/table/Car_campare.tex <==
\begin{table*}[t]
\renewcommand\arraystretch{1.5}
\caption{Rollout MSE on ParticleCar. L(low-speed), M(medium-speed), and H(high-speed) represent three speed intervals: 10-30, 30-70, and 70-100 }
\centering
\scalebox{0.69}{
\label{tab:car_compare}
\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
\bottomrule
\multicolumn{1}{c|}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{t = 30}} & \multicolumn{3}{c|}{\textbf{t = 60}} & \multicolumn{3}{c}{\textbf{t = 90}}\\
\cline{2-10}
& \textbf{\textit{L}} & \textbf{\textit{M}} & \textbf{\textit{H}} & \textbf{\textit{L}} & \textbf{\textit{M}} & \textbf{\textit{H}} & \textbf{\textit{L}} & \textbf{\textit{M}} & \textbf{\textit{H}} \\
\hline
\textbf{GNS} & \textbf{1.12$\pm$0.45} & 3.67$\pm$0.85 & 5.08$\pm$1.67 & \textbf{6.79/1.13} & 12.88$\pm$3.71 & 20.32$\pm$5.19 & \textbf{8.97$\pm$1.01} & 34.33$\pm$4.92 & 61.39$\pm$5.09 \\
\textbf{SGNN} & \textbf{1.19$\pm$0.79} & 5.21$\pm$1.47 & 8.01$\pm$2.59 & \textbf{4.51$\pm$1.52} & 15.29$\pm$3.45 & 23.53$\pm$5.04 & \textbf{8.81$\pm$2.35} & 32.61$\pm$2.27 & 57.16$\pm$7.02 \\
\textbf{HGNN} & \textbf{13.41$\pm$2.66} & 15.59$\pm$3.54 & 20.23$\pm$1.67 & \textbf{34.78$\pm$5.13} & 45.01$\pm$7.21 & 50.87$\pm$6.48 & \textbf{71.38$\pm$8.01} & 113.03$\pm$9.79 & 217.65$\pm$13.39 \\
\textbf{LGNN} & \textbf{3.42$\pm$0.45} & 4.31$\pm$2.32 & 7.43$\pm$1.99 & \textbf{8.54$\pm$2.70} & 15.30$\pm$6.15 & 25.11$\pm$6.04 & \textbf{21.97$\pm$4.08} & 75.29$\pm$10.84 & 97.26$\pm$5.75 \\
\bottomrule
\end{tabular}
}
    \vskip -0.1in
\end{table*}



==> ICIC/table/Car_mse.tex <==
\begin{table}[t]
\renewcommand\arraystretch{1.5}
\caption{Rollout MSE on ParticleCar}
\label{tab:ParticleCar}
\centering


\begin{tabular}{l c c c c}
\toprule
\ & \textbf{t=10} & \textbf{t=20}  & \textbf{t=40} & \textbf{t=100} \\ 
\bottomrule
\rowcolor{gray!20}\textbf{GNS}  & 0.11$\pm$0.06 & 0.38$\pm$0.07 & 1.46$\pm$0.17 & 9.91$\pm$0.79 \\
\toprule
\textbf{SGNN} & 0.81$\pm$0.08 & 1.04$\pm$0.41 & 1.24$\pm$0.19 & 9.34$\pm$2.79 \\
\textbf{$\Delta$} & \textcolor{red}{0.70} $\uparrow$ & \textcolor{red}{0.66} $\uparrow$ & \textcolor{green}{-0.22} $\downarrow$ & \textcolor{green}{-0.57} $\downarrow$ \\
\hline
\textbf{HGNN} & 3.73$\pm$0.44 & 11.97$\pm$2.44 & 22.31$\pm$4.02 & 86.45$\pm$5.16 \\
\textbf{$\Delta$} & \textcolor{red}{3.62} $\uparrow$ & \textcolor{red}{11.59} $\uparrow$ & \textcolor{red}{20.85} $\uparrow$ & \textcolor{red}{76.54} $\uparrow$ \\
\hline
\textbf{LGNN} & 0.41$\pm$0.23 & 1.03$\pm$0.64 & 15.32$\pm$2.56 & 23.47$\pm$4.32 \\
\textbf{$\Delta$} & \textcolor{red}{0.30} $\uparrow$ & \textcolor{red}{0.65} $\uparrow$ & \textcolor{red}{13.86} $\uparrow$ & \textcolor{red}{13.56} $\uparrow$ \\
\toprule
\end{tabular}



\end{table}

==> ICIC/table/comparison.tex <==

\begin{table*}[t]
\renewcommand\arraystretch{1.1}
\caption{Comparison across related datasets. ``--'' means is not officially reported in the corresponding paper.}
\label{tab:comparision}
\definecolor{mygray}{rgb}{0.8, 0.8, 0.8} % 浅灰色

\centering
\scalebox{0.78}{
\begin{tabular}{@{}lccc|cccc|cc|cc@{}}
\toprule
\hline
\textbf{Dataset} & \multicolumn{3}{c}{\textbf{Dimensions}}  & \multicolumn{4}{c}{ \textbf{The Number of}} & \multicolumn{2}{c}{\textbf{Force}}& \multicolumn{2}{c}{\textbf{Dynamics}} \\



 &1D &2D&3D  & Trajectories & Time-steps  & Scenarios & Objects & Static  & Variable & Single&Multi  \\
 \hline
\bottomrule
RigidFall\cite{RigidFall} & \texttimes & \texttimes & \checkmark & 5000 & 120& 1 & 3 & \checkmark & \texttimes  &\checkmark &\texttimes \\
FLAGSIMPLE \cite{GNS} & \texttimes & \checkmark & \texttimes  & 800 & 200& 1 & 1 & \texttimes & \texttimes  & \checkmark &\texttimes  \\
CYLINDERFLOW \cite{GNS}  &\texttimes & \checkmark & \texttimes & 800 & 400& 1 & 1 & \texttimes & \texttimes & \checkmark &\texttimes \\
AIRFOIL\cite{Mesh/iclr/PfaffFSB21}     &\texttimes & \checkmark & \texttimes & 1000 & 150 & 1 & 1 &\texttimes & \texttimes & \checkmark &\texttimes \\
Cub-Toss \cite{Cubtoss}    &\texttimes & \texttimes & \checkmark  & 10000 & 80 & 1 & 1 &\texttimes & \texttimes & \checkmark &\texttimes \\
INFLATINGFONT \cite{BMS}   &\texttimes & \checkmark & \texttimes  & 1000 & 100 & 1 & 1 &\texttimes & \texttimes  & \checkmark &\texttimes  \\
\hline
N-Pendulum \cite{LGNN} &\texttimes & \checkmark & \texttimes & 100 & 100 & 5 &1 &\checkmark & \texttimes  &\checkmark &\texttimes\\
N-Spring \cite{HGNN}  &\texttimes & \checkmark & \texttimes & 100 & 100 & 5 & 1 &\checkmark & \texttimes  &\checkmark &\texttimes\\
Spring-ball \cite{LGNN} &\texttimes & \checkmark & \texttimes & 1000 & 50 & 1 & 2 &\texttimes &\checkmark  &\texttimes &\checkmark\\

MD17 \cite{MD17}   &\texttimes & \checkmark & \texttimes & 2000 & 500 & 1 & 2  & \texttimes &\checkmark  &\texttimes &\checkmark\\
CMU\cite{CMU} &\texttimes & \texttimes & \checkmark  & 86 & 100 & 1 & 1 &\texttimes &\checkmark  &\texttimes &\checkmark \\
Cavity Flow\cite{Lid}   &\texttimes & \checkmark & \texttimes & 1000 & 60 & 1 & 1 &\texttimes &\checkmark  &\texttimes &\checkmark\\
Granular flow \cite{boundary} &\texttimes & \texttimes & \checkmark  & 365 & 250 & 2 & 1 &\checkmark & \texttimes  &\checkmark &\texttimes\\
Kubric MOVi-A\cite{Kubric}  &\texttimes & \texttimes & \checkmark  & -- & -- & 1 & 3 &\checkmark & \texttimes  &\checkmark &\texttimes\\
ROPE \cite{rope} &\texttimes &\checkmark &\texttimes  & 10000 & 160 & 1 & 1 &\checkmark & \texttimes  &\checkmark &\texttimes\\
\hline
3 mode system \cite{3}  &\texttimes &\checkmark &\texttimes   & 10500 & 180 & 1 & 3  &\checkmark & \texttimes  &\checkmark &\texttimes\\
Bouncing ball \cite{3}  &\checkmark &\texttimes  &\texttimes   & 1100 & 100 & 1 & 1  &\checkmark & \texttimes  &\checkmark &\texttimes\\
Simulated Cloth \cite{cloth} &\texttimes &\checkmark  &\checkmark   & 1050 & 160 & 1 & 1 & \texttimes &\checkmark   &\checkmark &\texttimes\\
Deformable Plate \cite{sensor} &\texttimes &\texttimes  &\checkmark   & 675 & 50 & 1 & 1 &\checkmark &\texttimes    &\checkmark &\texttimes\\
\hline
\textbf{MBDS(ours)} & \textbf{\checkmark} &\textbf{\checkmark} &\textbf{\checkmark} & \textbf{15000} & \textbf{200} & \textbf{8} & \textbf{32(Ave)} &\textbf{\checkmark} & \textbf{\checkmark }&\textbf{\checkmark} &\textbf{\checkmark}  \\
 \hline
\bottomrule
\end{tabular}
}
\end{table*}

==> ICIC/table/cubli.tex <==
\begin{table}[t]
\renewcommand\arraystretch{1.5}
\caption{Rollout MSE on SimpleCubli}
\label{tab:SimpleCubli}
\centering
\begin{tabular}{l c c c c}
\toprule
\ & \textbf{t=10} & \textbf{t=20}  & \textbf{t=40} & \textbf{t=100} \\ 
\bottomrule
\rowcolor{gray!20}\textbf{GNS}  & 0.57$\pm$0.05 & 1.27$\pm$0.14 & 1.89$\pm$0.22 & 9.42$\pm$1.98 \\
\toprule
\textbf{SGNN} & 0.43$\pm$0.37 & 2.34$\pm$1.37 & 8.32$\pm$2.98 & 119.89$\pm$10.75 \\
\textbf{$\Delta$} & \textcolor{green}{-0.14} $\downarrow$ & \textcolor{red}{1.07} $\uparrow$ & \textcolor{red}{6.43} $\uparrow$ & \textcolor{red}{110.47} $\uparrow$ \\
\hline
\textbf{HGNN} & 6.69$\pm$1.03 & 9.37$\pm$0.26 & 19.01$\pm$2.45 & 34.71$\pm$7.63 \\
\textbf{$\Delta$} & \textcolor{red}{6.12} $\uparrow$ & \textcolor{red}{8.10} $\uparrow$ & \textcolor{red}{17.12} $\uparrow$ & \textcolor{red}{25.29} $\uparrow$ \\
\hline
\textbf{LGNN} & 4.32$\pm$0.98 & 12.10$\pm$1.34 & 24.32$\pm$6.45 & 41.45$\pm$8.98 \\
\textbf{$\Delta$} & \textcolor{red}{3.75} $\uparrow$ & \textcolor{red}{10.83} $\uparrow$ & \textcolor{red}{22.43} $\uparrow$ & \textcolor{red}{32.03} $\uparrow$ \\
\toprule
\end{tabular}


\end{table}

==> ICIC/table/ladder.tex <==
\begin{table}[t]
\renewcommand\arraystretch{1.5}
\caption{Rollout MSE on 3-Ladder. }
\label{tab:ladder}
\centering
\begin{tabular}{l c c c c}
\toprule
\ & \textbf{t=10} & \textbf{t=20}  & \textbf{t=40} & \textbf{t=100} \\ 
\bottomrule
\rowcolor{gray!20}\textbf{GNS}  & 0.77$\pm$0.01 & 1.01$\pm$0.14 & 3.56$\pm$0.12 & 12.42$\pm$0.18 \\
\toprule
\textbf{SGNN} & 0.14$\pm$0.01 & 0.62$\pm$0.03 & 1.46$\pm$0.33 & 9.31$\pm$0.16 \\
\textbf{$\Delta$} & \textcolor{green}{-0.63} $\downarrow$ & \textcolor{green}{-0.39} $\downarrow$ & \textcolor{green}{-2.10} $\downarrow$ & \textcolor{green}{-3.11} $\downarrow$ \\
\hline
\textbf{HGNN} & 0.21$\pm$0.03 & 0.72$\pm$0.26 & 1.67$\pm$0.52 & 10.56$\pm$0.63 \\
\textbf{$\Delta$} & \textcolor{green}{-0.56} $\downarrow$ & \textcolor{green}{-0.29} $\downarrow$ & \textcolor{green}{-1.89} $\downarrow$ & \textcolor{green}{-1.86} $\downarrow$ \\
\hline
\textbf{LGNN} & 0.81$\pm$0.32 & 1.03$\pm$0.17 & 1.50$\pm$0.89 & 8.87$\pm$1.74 \\
\textbf{$\Delta$} & \textcolor{red}{0.04} $\uparrow$ & \textcolor{red}{0.02} $\uparrow$ & \textcolor{green}{-2.06} $\downarrow$ & \textcolor{green}{-3.55} $\downarrow$ \\
\toprule
\end{tabular}

\end{table}


==> ICIC/table/mujoco.tex <==

\begin{table}[h]
\caption{Particle Parameters}
\label{tab:mujoco}
\begin{center}
\begin{tabular}{c|c|c|c}
\hline
\textbf{Constant} & \textbf{\textit{Symbol}} & \textbf{\textit{Value}} & \textbf{\textit{Units}} \\
\hline
mass & \( m \) & 1 & kg \\
\hline
inertia & \( I \) & \( 6.17 \times 10^{-4} \) & kg\(\cdot\)m\(^2\) \\
\hline
force & \( F \) & (various) & N \\
\hline
gravity & \( g \) & 9.81 & m/s\(^2\) \\
\hline
friction coefficient & \( \mu \) & \(4.3\times 10^{-1}\) & (none) \\
\hline

damping ratio & \( \zeta \) & \(2.2 \times 10^{-2}\) & (none) \\
\hline
time-step & \( \Delta t \) & \( 2 \times 10^{-2} \) & s \\
\hline
\end{tabular}
\label{tab:die_roll_parameters}
   
\end{center}
 \vskip -0.4in
\end{table}


==> ICIC/table/new_result.tex <==
\begin{table*}[t]
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{8pt}

\centering
    \caption{Comparative experiment results. \textbf{Bold} indicates the method with optimal performance. \underline{Underline} denotes the method with second-best performance. Some standard deviations are marked as 0.00 due to being too small to effectively represent.}
    \label{tab:main_result}
    \scalebox{0.85}{     

    \begin{tabular}{c|l|ccccc}
        \hline
               \multicolumn{2}{c|}{Senario} & \multirow{2}{*}{ParticleCar} &  \multirow{2}{*}{6-Pendulum} & \multirow{2}{*}{SimpleCubli} &\multirow{2}{*}{3-Ladder}&\multirow{2}{*}{BallDrop}\\
        \cline{1-2}
        Time & Methods   \\
        \hline
        \multirow{4}{*}{\rotatebox[origin=c]{90}{t=10}} 
        \scriptsize\multirow{4}{*}{\rotatebox[origin=c]{90}{(MSE $\times 10^{0}$)}}
         & GNS  & \textbf{0.11$\pm$0.06} & \textbf{0.21$\pm$0.05} & \underline{0.57$\pm$0.05}  & 0.77$\pm$0.01 & 0.23$\pm$0.02 \\
         & SGNN & 0.81$\pm$0.08 & \underline{0.45$\pm$0.08} & \textbf{0.43$\pm$0.37} & \textbf{0.14$\pm$0.01} & \underline{0.33$\pm$0.08} \\
         & HGNN & 3.73$\pm$0.44 & 0.61$\pm$0.07 & 6.69$\pm$1.03 & \underline{0.21$\pm$0.03} &0.17$\pm$0.06 \\
         & LGNN & \underline{0.41}$\pm$0.23 & 0.87$\pm$0.26 & 4.32$\pm$0.98 & 0.81$\pm$0.32 & \textbf{0.16$\pm$0.03} \\
        % & MDGS (Ours)  & \textbf{0.84$\pm$0.28}  & \textbf{1.76$\pm$0.63}    & \textbf{2.08$\pm$0.24}   &  \textbf{0.84$\pm$0.04}   \\
        \hline
        \multirow{4}{*}{\rotatebox[origin=c]{90}{t=20}} 
        \scriptsize\multirow{4}{*}{\rotatebox[origin=c]{90}{(MSE $\times 10^{0}$)}}
             & GNS  & \textbf{0.38$\pm$0.07}     & \textbf{0.39$\pm$0.15}     &\textbf{1.27$\pm$0.14}     & \underline{1.01$\pm$0.14} & \textbf{0.26$\pm$0.01} \\
             & SGNN & 1.05$\pm$0.41              & \underline{1.29$\pm$0.35}  & \underline{2.34$\pm$1.27} & \textbf{0.62$\pm$0.03} &0.41$\pm$0.12 \\
             & HGNN & 11.97$\pm$2.44               & 1.33$\pm$0.28              & 9.37$\pm$2.06             & 0.72$\pm$0.26 & \underline{0.35$\pm$0.03} \\
             & LGNN & \underline{1.03$\pm$0.64}     & 1.32$\pm$0.54              & 12.10$\pm$1.34          & 1.03$\pm$0.17 & 0.39$\pm$0.05 \\
        % & MDGS (Ours)  & \textbf{0.84$\pm$0.28}  & \textbf{1.76$\pm$0.63}    & \textbf{2.08$\pm$0.24}   &  \textbf{0.84$\pm$0.04}   \\
        \hline
                \multirow{4}{*}{\rotatebox[origin=c]{90}{t=40}} 
                \scriptsize\multirow{4}{*}{\rotatebox[origin=c]{90}{(MSE $\times 10^{1}$)}}
         & GNS  & \underline{0.15$\pm$0.01} & \textbf{0.11$\pm$0.02} & \textbf{0.19$\pm$0.02} & 0.37$\pm$0.01 & \textbf{0.03$\pm$0.00} \\
         & SGNN & \textbf{0.12$\pm$0.02} & 0.50$\pm$0.14 & \underline{0.83$\pm$0.29} & \textbf{0.14$\pm$0.03} & 0.08$\pm$0.01 \\
         & HGNN & 2.31$\pm$0.40 & \underline{0.16$\pm$0.06} & 1.90$\pm$0.24 & 0.17$\pm$0.05 & 0.07$\pm$0.02 \\
         & LGNN & 1.53$\pm$0.26 & 0.21$\pm$0.07 & 2.43$\pm$0.64 & \underline{0.15$\pm$0.09} & \underline{0.04$\pm$0.00} \\
        % & MDGS (Ours)  & \textbf{0.17$\pm$0.08} & \textbf{0.24 $\pm$0.06}    & \textbf{0.31$\pm$0.03}   & \textbf{0.15$\pm$0.04}   \\
        \hline

                        \multirow{4}{*}{\rotatebox[origin=c]{90}{t=100}} 
                    \scriptsize\multirow{4}{*}{\rotatebox[origin=c]{90}{(MSE $\times 10^{1}$)}} 
         & GNS  & \underline{0.99$\pm$0.07} & 2.16$\pm$0.52 & \textbf{0.94$\pm$0.19} & 1.24$\pm$0.01 & \textbf{0.21$\pm$0.08} \\
         & SGNN & \textbf{0.93$\pm$0.27} & 2.64$\pm$0.44 & 11.98$\pm$1.07 & \underline{0.93$\pm$0.01} & \underline{0.34$\pm$0.23} \\
         & HGNN & 8.64$\pm$0.51 & \underline{0.78$\pm$0.39} & \underline{3.47$\pm$0.76} & 1.05$\pm$0.06 & 0.45$\pm$0.11 \\
         & LGNN & 2.34$\pm$0.43 & \textbf{0.28$\pm$0.08} & 4.14$\pm$0.89 & \textbf{0.88$\pm$0.17} & 0.64$\pm$0.06 \\
        % & MDGS (Ours)  & \textbf{0.05$\pm$0.01}   & \textbf{0.06$\pm$0.01}    & \textbf{0.09$\pm$0.01}  & \textbf{0.04$\pm$0.01} \\
        \hline
    
    \end{tabular}
}
    \vskip -0.1in


\end{table*}


==> ICIC/table/pendulum.tex <==
\begin{table}[t]
 \vspace{3pt}
\renewcommand\arraystretch{1.5}
\caption{Rollout MSE on 6-Pendulum}
\label{tab:6-pendulum}
\centering
\begin{tabular}{l c c c c}
\toprule
\ & \textbf{t=10} & \textbf{t=20}  & \textbf{t=40} & \textbf{t=100} \\ 
\bottomrule
\rowcolor{gray!20}\textbf{GNS}  & 0.21$\pm$0.05 & 0.39$\pm$0.15 & 1.08$\pm$0.20 & 21.63$\pm$5.26 \\
\toprule
\textbf{SGNN} & 0.45$\pm$0.08 & 1.29$\pm$0.35 & 4.96$\pm$1.41 & 26.37$\pm$4.39 \\
\textbf{$\Delta$} & \textcolor{red}{0.24} $\uparrow$ & \textcolor{red}{0.90} $\uparrow$ & \textcolor{red}{3.88} $\uparrow$ & \textcolor{red}{4.74} $\uparrow$ \\
\hline
\textbf{HGNN} & 0.61$\pm$0.07 & 1.33$\pm$0.28 & 1.62$\pm$0.61 & 7.84$\pm$3.90 \\
\textbf{$\Delta$} & \textcolor{red}{0.40} $\uparrow$ & \textcolor{red}{0.94} $\uparrow$ & \textcolor{red}{0.54} $\uparrow$ & \textcolor{green}{-13.79} $\downarrow$ \\
\hline
\textbf{LGNN} & 0.87$\pm$0.26 & 1.29$\pm$0.54 & 1.95$\pm$0.72 & 2.79$\pm$0.79 \\
\textbf{$\Delta$} & \textcolor{red}{0.66} $\uparrow$ & \textcolor{red}{0.90} $\uparrow$ & \textcolor{red}{0.87} $\uparrow$ & \textcolor{green}{-18.84} $\downarrow$ \\
\toprule
\end{tabular}

\end{table}

==> ICIC/table/reseult.tex <==
\begin{table*}[t]
\renewcommand\arraystretch{1.5}
\caption{Rollout MSE $(\times 10^{-2})$ on MBDS when \( t \)=1}
\label{tab:result:1}
\centering
\scalebox{0.77}{
\begin{tabular}{l c c c c c c c c }
\toprule
\ & \textbf{ParticleCar} & \textbf{6-pundulum}  & \textbf{5-pendulum} & \textbf{3-ladder} &\textbf{2-ladder} & \textbf{SimpleCubli}  & \textbf{BallDrop} & \textbf{BallScroll} \\ 
\bottomrule
\rowcolor{gray!20} \textbf{GNS}    &0.72$ \pm$0.60   &1.44$ \pm$ 0.34    &0.39$ \pm$ 0.23    &0.41$\pm$0.04  &0.29$ \pm$0.16    &2.23$ \pm$0.14 &0.13$ \pm$0.01   &0.17 $\pm$ 0.01     \\
\toprule
\textbf{SGNN}   &1.93 $\pm$ 0.28     &1.32$\pm$ 0.65   &1.24$\pm$1.92   &0.83$\pm$0.19   &0.54$\pm$0.10   &1.34$\pm$0.44  &0.45$\pm$0.09   &0.23$\pm$0.02   \\
\textbf{$\Delta$} & \textcolor{red}{1.21} $\uparrow$ & \textcolor{green}{-0.12} $\downarrow$ & \textcolor{red}{0.85} $\uparrow$ & \textcolor{red}{0.42} $\uparrow$ & \textcolor{red}{0.25} $\uparrow$ & \textcolor{green}{-0.89} $\downarrow$ & \textcolor{red}{0.32} $\uparrow$ & \textcolor{red}{0.06} $\uparrow$ \\
\hline
\textbf{HGNN}    &2.89$\pm$1.12    &1.50$\pm$1.27   &1.31$\pm$1.74   &0.95$\pm$0.27   &0.78$\pm$0.20   &2.34$\pm$0.31   &0.51$\pm$0.23  &0.15$\pm$0.12   \\
\textbf{$\Delta$} & \textcolor{red}{2.17} $\uparrow$ & \textcolor{red}{0.06} $\uparrow$ & \textcolor{red}{0.92} $\uparrow$ & \textcolor{red}{0.54} $\uparrow$ & \textcolor{red}{0.49} $\uparrow$ & \textcolor{red}{0.11} $\uparrow$ & \textcolor{green}{-0.30} $\downarrow$ & \textcolor{green}{-0.02} $\downarrow$ \\
\hline
\textbf{LGNN}   &1.74$\pm$0.42   &1.58$\pm$1.04     &1.11$\pm$0.39   &4.36$\pm$1.33  &0.45$\pm$0.23   &3.20$\pm$0.52    &0.25$\pm$0.14 & /0.14$\pm$0.03   \\
\textbf{$\Delta$} & \textcolor{red}{1.02} $\uparrow$ & \textcolor{green}{-0.04} $\downarrow$ & \textcolor{red}{0.72} $\uparrow$ & \textcolor{red}{3.95} $\uparrow$ & \textcolor{red}{0.16} $\uparrow$ & \textcolor{red}{0.97} $\uparrow$ & \textcolor{red}{0.12} $\uparrow$ & \textcolor{green}{-0.03} $\downarrow$ \\
\toprule
\end{tabular}
}
    \vskip -0.1in
\end{table*}

==> ICIC/table/result50.tex <==
\begin{table*}[h]
\renewcommand\arraystretch{1.5}

\caption{Rollout MSE on MBD when \( t \)=50}
\label{tab:result:50}
\centering
\scalebox{0.78}{
\begin{tabular}{l c c c c c c c c }
\toprule
\ & \textbf{ParticleCar} & \textbf{6-pundulum}  & \textbf{5-pendulum} & \textbf{3-ladder} &\textbf{2-ladder} & \textbf{SimpleCubli}  & \textbf{BallDrop} & \textbf{BallScroll} \\ 
\bottomrule
\rowcolor{gray!20}\textbf{GNS}    &2.98$\pm$0.24   &1.94$\pm$0.29    &1.75$\pm$1.43    &6.75$\pm$2.94  &5.64$\pm$0.87    &2.34$\pm$0.34 &1.75$\pm$1.43   &0.37$\pm$0.21     \\
\toprule
\textbf{SGNN}   &2.56$\pm$0.48     &8.32$\pm$2.65   &6.24$\pm$1.92   &1.05$\pm$0.79   &1.04$\pm$0.49   &5.64$\pm$1.54  &2.65$\pm$1.43   &0.53$\pm$0.12   \\
\textbf{$\Delta$} & \textcolor{green}{-0.42} $\downarrow$ & \textcolor{red}{6.38} $\uparrow$ & \textcolor{red}{4.49} $\uparrow$ & \textcolor{green}{-5.70} $\downarrow$ & \textcolor{green}{-4.60} $\downarrow$ & \textcolor{red}{3.30} $\uparrow$ & \textcolor{red}{0.90} $\uparrow$ & \textcolor{red}{0.16} $\uparrow$ \\
\hline
\textbf{HGNN}    &29.13$\pm$3.72    &2.73$\pm$1.27   &2.67$\pm$0.34   &3.05$\pm$1.02   &2.94$\pm$0.86  &15.24$\pm$1.82   &1.45$\pm$1.43  &0.74$\pm$0.02   \\
\textbf{$\Delta$} & \textcolor{red}{26.15} $\uparrow$ & \textcolor{red}{0.79} $\uparrow$ & \textcolor{red}{0.92} $\uparrow$ & \textcolor{green}{-3.70} $\downarrow$ & \textcolor{green}{-2.70} $\downarrow$ & \textcolor{red}{12.90} $\uparrow$ & \textcolor{green}{-0.30} $\downarrow$ & \textcolor{red}{0.37} $\uparrow$ \\
\hline
\textbf{LGNN}   &8.87$\pm$2.43   &1.90$\pm$1.18     &1.82$\pm$0.56   &2.17$\pm$0.75  &1.74$\pm$0.37   &21.97$\pm$1.49    &4.75$\pm$1.43 &0.32$\pm$0.01   \\
\textbf{$\Delta$} & \textcolor{red}{5.89} $\uparrow$ & \textcolor{green}{-0.04} $\downarrow$ & \textcolor{red}{0.07} $\uparrow$ & \textcolor{green}{-4.58} $\downarrow$ & \textcolor{green}{-3.90} $\downarrow$ & \textcolor{red}{19.63} $\uparrow$ & \textcolor{red}{3.00} $\uparrow$ & \textcolor{green}{-0.05} $\downarrow$ \\
\toprule
\end{tabular}
}
    \vskip -0.1in
\end{table*}

==> ICIC/table/tamplet.tex <==
\begin{table}[t]
\renewcommand\arraystretch{1.5}
\caption{Rollout MSE on 3-Ladder. }
\label{tab:ladder}
\centering
\begin{tabular}{l c c c c}
\toprule
\ & \textbf{t=10} & \textbf{t=20}  & \textbf{t=40} & \textbf{t=100} \\ 
\bottomrule
\rowcolor{gray!20}\textbf{GNS}  & 0.77$\pm$0.01 & 1.01$\pm$0.14 & 3.56$\pm$0.12 & 12.42$\pm$0.18 \\
\toprule
\textbf{SGNN} & 0.14$\pm$0.01 & 0.62$\pm$0.03 & 1.46$\pm$0.33 & 9.31$\pm$0.16 \\
\textbf{$\Delta$} & \textcolor{green}{-0.63} $\downarrow$ & \textcolor{green}{-0.39} $\downarrow$ & \textcolor{green}{-2.10} $\downarrow$ & \textcolor{green}{-3.11} $\downarrow$ \\
\hline
\textbf{HGNN} & 0.21$\pm$0.03 & 0.72$\pm$0.26 & 1.67$\pm$0.52 & 10.56$\pm$0.63 \\
\textbf{$\Delta$} & \textcolor{green}{-0.56} $\downarrow$ & \textcolor{green}{-0.29} $\downarrow$ & \textcolor{green}{-1.89} $\downarrow$ & \textcolor{green}{-1.86} $\downarrow$ \\
\hline
\textbf{LGNN} & 0.81$\pm$0.32 & 1.03$\pm$0.17 & 1.50$\pm$0.89 & 8.87$\pm$1.74 \\
\textbf{$\Delta$} & \textcolor{red}{0.04} $\uparrow$ & \textcolor{red}{0.02} $\uparrow$ & \textcolor{green}{-2.06} $\downarrow$ & \textcolor{green}{-3.55} $\downarrow$ \\
\toprule
\end{tabular}

\end{table}


==> table/Car_mse.tex <==
\begin{table}[t]
\renewcommand\arraystretch{1.5}
\caption{Rollout MSE on ParticleCar}
\label{tab:ParticleCar}
\centering


\begin{tabular}{l c c c c}
\toprule
\ & \textbf{t=10} & \textbf{t=20}  & \textbf{t=40} & \textbf{t=100} \\ 
\bottomrule
\rowcolor{gray!20}\textbf{GNS}  & 0.11$\pm$0.06 & 0.38$\pm$0.07 & 1.46$\pm$0.17 & 9.91$\pm$0.79 \\
\toprule
\textbf{SGNN} & 0.81$\pm$0.08 & 1.04$\pm$0.41 & 1.24$\pm$0.19 & 9.34$\pm$2.79 \\
\textbf{$\Delta$} & \textcolor{red}{0.70} $\uparrow$ & \textcolor{red}{0.66} $\uparrow$ & \textcolor{green}{-0.22} $\downarrow$ & \textcolor{green}{-0.57} $\downarrow$ \\
\hline
\textbf{HGNN} & 3.73$\pm$0.44 & 11.97$\pm$2.44 & 22.31$\pm$4.02 & 86.45$\pm$5.16 \\
\textbf{$\Delta$} & \textcolor{red}{3.62} $\uparrow$ & \textcolor{red}{11.59} $\uparrow$ & \textcolor{red}{20.85} $\uparrow$ & \textcolor{red}{76.54} $\uparrow$ \\
\hline
\textbf{LGNN} & 0.41$\pm$0.23 & 1.03$\pm$0.64 & 15.32$\pm$2.56 & 23.47$\pm$4.32 \\
\textbf{$\Delta$} & \textcolor{red}{0.30} $\uparrow$ & \textcolor{red}{0.65} $\uparrow$ & \textcolor{red}{13.86} $\uparrow$ & \textcolor{red}{13.56} $\uparrow$ \\
\toprule
\end{tabular}



\end{table}

==> table/cubli.tex <==
\begin{table}[t]
\renewcommand\arraystretch{1.5}
\caption{Rollout MSE on SimpleCubli}
\label{tab:SimpleCubli}
\centering
\begin{tabular}{l c c c c}
\toprule
\ & \textbf{t=10} & \textbf{t=20}  & \textbf{t=40} & \textbf{t=100} \\ 
\bottomrule
\rowcolor{gray!20}\textbf{GNS}  & 0.57$\pm$0.05 & 1.27$\pm$0.14 & 1.89$\pm$0.22 & 9.42$\pm$1.98 \\
\toprule
\textbf{SGNN} & 0.43$\pm$0.37 & 2.34$\pm$1.37 & 8.32$\pm$2.98 & 119.89$\pm$10.75 \\
\textbf{$\Delta$} & \textcolor{green}{-0.14} $\downarrow$ & \textcolor{red}{1.07} $\uparrow$ & \textcolor{red}{6.43} $\uparrow$ & \textcolor{red}{110.47} $\uparrow$ \\
\hline
\textbf{HGNN} & 6.69$\pm$1.03 & 9.37$\pm$0.26 & 19.01$\pm$2.45 & 34.71$\pm$7.63 \\
\textbf{$\Delta$} & \textcolor{red}{6.12} $\uparrow$ & \textcolor{red}{8.10} $\uparrow$ & \textcolor{red}{17.12} $\uparrow$ & \textcolor{red}{25.29} $\uparrow$ \\
\hline
\textbf{LGNN} & 4.32$\pm$0.98 & 12.10$\pm$1.34 & 24.32$\pm$6.45 & 41.45$\pm$8.98 \\
\textbf{$\Delta$} & \textcolor{red}{3.75} $\uparrow$ & \textcolor{red}{10.83} $\uparrow$ & \textcolor{red}{22.43} $\uparrow$ & \textcolor{red}{32.03} $\uparrow$ \\
\toprule
\end{tabular}


\end{table}

==> table/ladder.tex <==
\begin{table}[t]
\renewcommand\arraystretch{1.5}
\caption{Rollout MSE on 3-Ladder. }
\label{tab:ladder}
\centering
\begin{tabular}{l c c c c}
\toprule
\ & \textbf{t=10} & \textbf{t=20}  & \textbf{t=40} & \textbf{t=100} \\ 
\bottomrule
\rowcolor{gray!20}\textbf{GNS}  & 0.77$\pm$0.01 & 1.01$\pm$0.14 & 3.56$\pm$0.12 & 12.42$\pm$0.18 \\
\toprule
\textbf{SGNN} & 0.14$\pm$0.01 & 0.62$\pm$0.03 & 1.46$\pm$0.33 & 9.31$\pm$0.16 \\
\textbf{$\Delta$} & \textcolor{green}{-0.63} $\downarrow$ & \textcolor{green}{-0.39} $\downarrow$ & \textcolor{green}{-2.10} $\downarrow$ & \textcolor{green}{-3.11} $\downarrow$ \\
\hline
\textbf{HGNN} & 0.21$\pm$0.03 & 0.72$\pm$0.26 & 1.67$\pm$0.52 & 10.56$\pm$0.63 \\
\textbf{$\Delta$} & \textcolor{green}{-0.56} $\downarrow$ & \textcolor{green}{-0.29} $\downarrow$ & \textcolor{green}{-1.89} $\downarrow$ & \textcolor{green}{-1.86} $\downarrow$ \\
\hline
\textbf{LGNN} & 0.81$\pm$0.32 & 1.03$\pm$0.17 & 1.50$\pm$0.89 & 8.87$\pm$1.74 \\
\textbf{$\Delta$} & \textcolor{red}{0.04} $\uparrow$ & \textcolor{red}{0.02} $\uparrow$ & \textcolor{green}{-2.06} $\downarrow$ & \textcolor{green}{-3.55} $\downarrow$ \\
\toprule
\end{tabular}

\end{table}


==> table/pendulum.tex <==
\begin{table}[t]
 \vspace{3pt}
\renewcommand\arraystretch{1.5}
\caption{Rollout MSE on 6-Pendulum}
\label{tab:6-pendulum}
\centering
\begin{tabular}{l c c c c}
\toprule
\ & \textbf{t=10} & \textbf{t=20}  & \textbf{t=40} & \textbf{t=100} \\ 
\bottomrule
\rowcolor{gray!20}\textbf{GNS}  & 0.21$\pm$0.05 & 0.39$\pm$0.15 & 1.08$\pm$0.20 & 21.63$\pm$5.26 \\
\toprule
\textbf{SGNN} & 0.45$\pm$0.08 & 1.29$\pm$0.35 & 4.96$\pm$1.41 & 26.37$\pm$4.39 \\
\textbf{$\Delta$} & \textcolor{red}{0.24} $\uparrow$ & \textcolor{red}{0.90} $\uparrow$ & \textcolor{red}{3.88} $\uparrow$ & \textcolor{red}{4.74} $\uparrow$ \\
\hline
\textbf{HGNN} & 0.61$\pm$0.07 & 1.33$\pm$0.28 & 1.62$\pm$0.61 & 7.84$\pm$3.90 \\
\textbf{$\Delta$} & \textcolor{red}{0.40} $\uparrow$ & \textcolor{red}{0.94} $\uparrow$ & \textcolor{red}{0.54} $\uparrow$ & \textcolor{green}{-13.79} $\downarrow$ \\
\hline
\textbf{LGNN} & 0.87$\pm$0.26 & 1.29$\pm$0.54 & 1.95$\pm$0.72 & 2.79$\pm$0.79 \\
\textbf{$\Delta$} & \textcolor{red}{0.66} $\uparrow$ & \textcolor{red}{0.90} $\uparrow$ & \textcolor{red}{0.87} $\uparrow$ & \textcolor{green}{-18.84} $\downarrow$ \\
\toprule
\end{tabular}

\end{table}

==> table/tamplet.tex <==
\begin{table}[t]
\renewcommand\arraystretch{1.5}
\caption{Rollout MSE on 3-Ladder. }
\label{tab:ladder}
\centering
\begin{tabular}{l c c c c}
\toprule
\ & \textbf{t=10} & \textbf{t=20}  & \textbf{t=40} & \textbf{t=100} \\ 
\bottomrule
\rowcolor{gray!20}\textbf{GNS}  & 0.77$\pm$0.01 & 1.01$\pm$0.14 & 3.56$\pm$0.12 & 12.42$\pm$0.18 \\
\toprule
\textbf{SGNN} & 0.14$\pm$0.01 & 0.62$\pm$0.03 & 1.46$\pm$0.33 & 9.31$\pm$0.16 \\
\textbf{$\Delta$} & \textcolor{green}{-0.63} $\downarrow$ & \textcolor{green}{-0.39} $\downarrow$ & \textcolor{green}{-2.10} $\downarrow$ & \textcolor{green}{-3.11} $\downarrow$ \\
\hline
\textbf{HGNN} & 0.21$\pm$0.03 & 0.72$\pm$0.26 & 1.67$\pm$0.52 & 10.56$\pm$0.63 \\
\textbf{$\Delta$} & \textcolor{green}{-0.56} $\downarrow$ & \textcolor{green}{-0.29} $\downarrow$ & \textcolor{green}{-1.89} $\downarrow$ & \textcolor{green}{-1.86} $\downarrow$ \\
\hline
\textbf{LGNN} & 0.81$\pm$0.32 & 1.03$\pm$0.17 & 1.50$\pm$0.89 & 8.87$\pm$1.74 \\
\textbf{$\Delta$} & \textcolor{red}{0.04} $\uparrow$ & \textcolor{red}{0.02} $\uparrow$ & \textcolor{green}{-2.06} $\downarrow$ & \textcolor{green}{-3.55} $\downarrow$ \\
\toprule
\end{tabular}

\end{table}

